FTTE: Enabling Federated and Resource-Constrained Deep Edge Intelligence

Federated learning (FL) enables collaborative model training across distributed devices while preserving data privacy, but deployment on resource-constrained edge nodes remains challenging due to limited memory, energy, and communication bandwidth. Traditional synchronous and asynchronous FL approaches further suffer from straggler induced delays and slow convergence in heterogeneous, large scale networks. We present FTTE (Federated Tiny Training Engine),a novel semi-asynchronous FL framework that uniquely employs sparse parameter updates and a staleness-weighted aggregation based on both age and variance of client updates. Extensive experiments across diverse models and data distributions - including up to 500 clients and 90% stragglers - demonstrate that FTTE not only achieves 81% faster convergence, 80% lower on-device memory usage, and 69% communication payload reduction than synchronous FL (eg.FedAVG), but also consistently reaches comparable or higher target accuracy than semi-asynchronous (eg.FedBuff) in challenging regimes. These results establish FTTE as the first practical and scalable solution for real-world FL deployments on heterogeneous and predominantly resource-constrained edge devices.

==> tables/algo.tex <==

\begin{wrapfigure}{L}{0.52\textwidth}
\begin{minipage}{0.5\textwidth}
\begin{algorithm}[H]
     \small
   \caption{Federated Tiny Training Engine} % %\lfbox[border-color=greeogin,border-width=1pt]{FedProx} %\cite{li2020federated},
   %\lfbox[border-color=red,border-width=1pt]{FedADAM}, and \lfbox[border-color=blue,border-width=1pt]{FedYogi} \cite{reddi2021adaptive}}
   \label{algo}
   $\text{For function and parameter description, refer to Table \ref{algo_desc}}$
   \vspace{0.3cm}
   
     \hspace{-1.2cm}$\textbf{Server Executes:}
  $
\begin{algorithmic}
  \STATE$ \text{Initialize }w_{g} \text{ with ImageNet pre-trained weights}$ 
   \STATE$ \text{Get memory constraint }M_{1,2,...,N} \text{ for all clients}$ 
   \STATE$ M_{min} = \min(M_1, M_2,..., M_N)$
   \STATE $\hat{w_g} \leftarrow \mathrm{ParamSelection}(w_g, m_{min})$
      \STATE $\text{Initialize } w_g \in R^d $
   \STATE $Reset(B)$
    \REPEAT
    \STATE$\text{Sample C available clients at random}$
    \STATE $\mathrm{ClientUpdate}(\hat{w_g})$
    \IF{recieve update from client i, $\hat{w^i}$}
    \STATE $B \leftarrow \hat{w^i} * Staleness(\hat{w^i})$
    \ENDIF
    \IF{B is full}
    \STATE $\hat{w_g} = Aggregate(B)$
    \STATE $Reset(B) $
    \ENDIF
    \UNTIL Convergence 
    \end{algorithmic}


\vspace{0.35cm}
\hspace{-0.00cm}$\textbf{ParamSelection(w, $M_{min}$)\cite{256}:}$
 \begin{algorithmic}
   \STATE$Ind^*(w)=\max\limits_{Ind(w)}(\Delta Acc_{Ind(w)}) \text{ s.t. } Mem.(w)\leq M_{min}$
   \IF{$Ind^j(w)$ in $Ind^*(w) \forall j \in Ind(w) $}
    \STATE Set $Freeze(w^j)=False$
    \ELSE
    \STATE Set $Freeze(w^j)=True$
    \ENDIF 
    \RETURN  $w$ 
\end{algorithmic}
    
 \vspace{0.35cm}
   \hspace{-1.2cm}$\textbf{ClientUpdate(w):}
  $
 \begin{algorithmic}
    \STATE $\text{Initialize }w_0 = w
    $
    \FOR{$\text{each local client iteration, $l=0,1,..,L-1$}$}
    \STATE $g_l = \nabla_{w}F_n(w_l)$
    %+ \lfbox[border-color=green,border-width=1pt]{\mu\frac{1}{2}||{w_i-w}||^2})$
      \STATE $w_{l+1} = w_{l} - \eta_l\text{ } g_l
      $
    \ENDFOR \\
    \RETURN  $w_{L}$ $\text{ to server}$
% \vspace{-10pt}
\end{algorithmic}
% \vspace{-5pt}
\end{algorithm}
\vspace{-5pt}
\end{minipage}
\end{wrapfigure}


==> tables/algo_2.tex <==
\begin{figure}[t]

    \begin{minipage}{0.48\textwidth}
    \begin{algorithm}[H]
     \small
   \caption{FTTE: Federated Tiny Training Engine} % %\lfbox[border-color=greeogin,border-width=1pt]{FedProx} %\cite{li2020federated},
   %\lfbox[border-color=red,border-width=1pt]{FedADAM}, and \lfbox[border-color=blue,border-width=1pt]{FedYogi} \cite{reddi2021adaptive}}
   \label{algo}
   \text{For parameter and function descriptions and function }
   \text{blocks, refer to Table \ref{algo_desc} and Algorithms \ref{algo2} and \ref{algo3}}\\
% \vspace{0.1cm}
    \centering
\begin{algorithmic}
\STATE$\textbf{Server Executes:}$
  \STATE$ \text{Initialize }w_{g} \text{ with ImageNet pre-trained weights}$ 
   \STATE$ \text{Get memory constraint }M_{1,2,...,N} \text{ for all clients}$ 
   \STATE$ M_{min} = \min(M_1, M_2,..., M_N)$
   \STATE $\hat{w_g} \leftarrow \mathrm{ParamSelection}(w_g, m_{min})$
      \STATE $\text{Initialize } w_g \in R^d $
   \STATE $Reset(B)$
    \REPEAT
    \STATE$\text{Sample C available clients at random}$
    \STATE $\mathrm{ClientUpdate}(\hat{w_g})$
    \IF{recieve update from client i, $\hat{w^i}$}
    \STATE $B \leftarrow \hat{w^i} * Staleness(\hat{w^i})$
    \ENDIF
    \IF{B is full}
    \STATE $\hat{w_g} = Aggregate(B)$
    \STATE $Reset(B) $
    \ENDIF
    \UNTIL Convergence 
    \end{algorithmic}
    \end{algorithm}
    \end{minipage}
    \hfill
\begin{minipage}{0.48\textwidth}
    \begin{algorithm}[H]
     \small
   \caption{Parameter Selection} % %\lfbox[border-color=greeogin,border-width=1pt]{FedProx} %\cite{li2020federated},
   %\lfbox[border-color=red,border-width=1pt]{FedADAM}, and \lfbox[border-color=blue,border-width=1pt]{FedYogi} \cite{reddi2021adaptive}}
   \label{algo2}
   \begin{algorithmic}
   \STATE$\textbf{ParamSelection(w, $M_{min}$)\cite{256}:}$
   \STATE$w^*=\max\limits_{w}(\Delta Acc_{w}) \text{ s.t. } Mem.(w)\leq M_{min}$
   \IF{$w_j$ in $w^* \forall w_j \in w $}
    \STATE Set $Freeze(w_j)=False$
    \ELSE
    \STATE Set $Freeze(w_j)=True$
    \ENDIF 
    \RETURN  $w$ 
\end{algorithmic}
    \end{algorithm}
\vfill
\begin{algorithm}[H]
     \small
   \caption{Client Updates} % %\lfbox[border-color=greeogin,border-width=1pt]{FedProx} %\cite{li2020federated},
   %\lfbox[border-color=red,border-width=1pt]{FedADAM}, and \lfbox[border-color=blue,border-width=1pt]{FedYogi} \cite{reddi2021adaptive}}
   \label{algo3}
   
 \begin{algorithmic}
 \STATE$\textbf{ClientUpdate(w):}$
    \STATE $\text{Initialize }w_0 = w
    $
    \FOR{$\text{each local client iteration, $l=0,1,..,L-1$}$}
    \STATE $g_l = \nabla_{w}F_n(w_l)$
    %+ \lfbox[border-color=green,border-width=1pt]{\mu\frac{1}{2}||{w_i-w}||^2})$
      \STATE $w_{l+1} = w_{l} - \eta_l\text{ } g_l
      $
    \ENDFOR \\
    \RETURN  $w_{L}$ $\text{ to server}$
% \vspace{-10pt}
\end{algorithmic}
    \end{algorithm}

    
    \end{minipage}
\end{figure}

==> tables/table1.tex <==

% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[b]
\caption{Description of parameter notations and functions used in Algorithm \ref{algo} and Section \ref{FTTE_sec}}
\label{algo_desc}
\centering
\footnotesize	
% \resizebox{\textwidth}{!}{
\begin{tabular}{cp{8cm}}
\hline
\textbf{\begin{tabular}[c]{@{}c@{}}Parameter \\ or Function\end{tabular}} & \hspace{2cm}\textbf{Description}                                              \\ \hline
\rowcolor[HTML]{EFEFEF} 
$w_g$                                                                     & All parameters of the global model                                \\
N                                                                         & Number of clients in the federated network                        \\
\rowcolor[HTML]{EFEFEF} 
$M_{1,2,...,N}$                                                           & Memory constraint of clients 1 to$ N  $                             \\
$\hat{w_g}$                                                               & Selected trainable parameters of the global model                 \\
\rowcolor[HTML]{EFEFEF} 
B                                                                         & Buffer of size determined by the user                             \\
C                                                                         & Fraction of clients randomly selected for training                \\
\rowcolor[HTML]{EFEFEF} 
$\hat{w^i}$                                                               & Trainable parameters of local model of client $i $                  \\
L                                                                         & Number of local epochs                                            \\
\rowcolor[HTML]{EFEFEF} 
$g_l$                                                                     & Gradient at local epoch $l  $                                       \\
$\eta_l$                                                                  & Local learning rate                                               \\
\rowcolor[HTML]{EFEFEF} 
$w^*$                                                                  & Selected trainable parameters from solving the optimization                           \\
$Staleness(\hat{w^i})$                                                     & Staleness of trainable parameters recieved from client $i  $        \\
\rowcolor[HTML]{EFEFEF} 
$Aggregate(B)    $                                                          & Federated aggregation of all model parameters in the buffer       \\
$Mem.(w)      $                                                             & Memory consumption of model when only parameters $w  $  are updated                    \\
\rowcolor[HTML]{EFEFEF} 
$\Delta Acc_w   $                                                               & Change in accuracy from updating only parameters $ w $ of the model                                 \\
$Reset(B)$                                                                  & Function that empties the buffer $B   $                             \\
\rowcolor[HTML]{EFEFEF} 
$Freeze(w_j) $                                                   & Function that freezes parameter $w_j$ based on the selection \\ \hline
\end{tabular}
\end{table}


==> tables/table2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[t]
\caption{Statistics of the different model architectures used in this paper.}
\label{stats}
\begin{tabular}{lccc}
\hline
\textbf{}                             & \multicolumn{1}{l}{\textbf{MCUNet}} & \multicolumn{1}{l}{\textbf{MobileNetV2}} & \multicolumn{1}{l}{\textbf{ProxylessNAS}} \\ \hline
\rowcolor[HTML]{EFEFEF} 
\textbf{Number of Parameters}         & 0.46 M                              & 0.29 M                                   & 0.36 M                                    \\
\textbf{MACs}                         & 22.5 M                              & 17.4 M                                   & 19.2 M                                    \\
\rowcolor[HTML]{EFEFEF} 
\textbf{Number of Layers}             & 42                                  & 52                                       & 61                                        \\
\textbf{Number of Blocks}             & 14                                  & 17                                       & 20                                        \\
\rowcolor[HTML]{EFEFEF} 
\textbf{Memory for Full Training}     & 218.85                              & 248.89                                   & 207.24                                    \\
\textbf{Memory for Last-Layer Update (TL)} & 42.23                               & 58.88                                    & 33.73                                     \\ 

% \textbf{Memory for FTTE with Sparse Update (Ours)} & 43.86                               & 60.1                                    & 33.96                                     \\
\hline
\end{tabular}
\end{table}

==> tables/table3.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\begin{tabular}{lccccc}
\hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{c}{\cellcolor[HTML]{EFEFEF}\textbf{Model}} & \textbf{Algorithm}                                                             & \textbf{Flowers-102}            & \textbf{Oxford-Pets} & \textbf{CIFAR-10} & \textbf{Skin Cancer} \\ \hline
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}                                   & \begin{tabular}[c]{@{}c@{}}Target \\ Acc.\end{tabular}                         & 51.8 \%                         & 58.23 \%             & 73.1 \%           & 73.1 \%              \\ \cline{2-6} 
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{FFFFFF}                                   & \textbf{FedAVG}                                                                & 6600 (x5.45)                    & 5000 (x3.98)         & 5000 (x7.09)      & 6000 (x5.04)         \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}                                   & \textbf{AsyncFL}                                                               &                                 &                      &                   &                      \\
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{FFFFFF}                                   & \textbf{FedBuff}                                                               & >10k (>x8.25)                   & >10k (>x7.97)        & 1497 (x2.12)      & 3443 (x2.89)         \\
\rowcolor[HTML]{FFFFFF} 
\multirow{-5}{*}{\cellcolor[HTML]{FFFFFF}MCUNet}           & \textbf{FTTE (Ours)}                                                           & 1211                            & 1255                 & 705               & 1189                 \\ \hline
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{FFFFFF}                                   & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}Target \\ Acc.\end{tabular} & \cellcolor[HTML]{EFEFEF}45.3 \% & 54.1 \%              & 70.1 \%           & 50.20 \%             \\ \cline{2-6} 
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}                                   & \textbf{FedAVG}                                                                & 4200 (x3.81)                    & 4400 (x4.87)         & 4600 (6.73)       & 5800 (x5.85)         \\
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{FFFFFF}                                   & \textbf{AsyncFL}                                                               &                                 &                      &                   &                      \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}                                   & \textbf{FedBuff}                                                               & >10k (x9.08)                    & >10k (>x11.07)       & >10k (>x14.64)    & 2591 (x2.61)         \\
\rowcolor[HTML]{EFEFEF} 
\multirow{-5}{*}{\cellcolor[HTML]{FFFFFF}MobileNetV2}      & \textbf{FTTE (Ours)}                                                           & 1101                            & 903                  & 683               & 991                  \\ \hline
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}                                   & \begin{tabular}[c]{@{}c@{}}Target \\ Acc.\end{tabular}                         & 53.8 \%                         & 58.6 \%              & 71.9 \%           & 48.91 \%             \\ \cline{2-6} 
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{FFFFFF}                                   & \textbf{FedAVG}                                                                & 6200 (x4.40)                    & 4600 (x4.18)         & 3800 (x5.95)      & 5800 (x6.75)         \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}                                   & \textbf{AsyncFL}                                                               & >10k (>x7.09)                   & Osc.                 &                   & >10k (>x11.64)       \\
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{FFFFFF}                                   & \textbf{FedBuff}                                                               & 1541 (x1.09)                    & >10k (>x9.08)        &                   & 3179 (x3.7)          \\
\rowcolor[HTML]{FFFFFF} 
\multirow{-5}{*}{\cellcolor[HTML]{FFFFFF}ProxylessNAS}     & \textbf{FTTE (Ours)}                                                           & 1409                            & 1101                 & 639               & 859                  \\ \hline
\end{tabular}
\end{table}

==> tables/table3_v2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\caption{Target accuracy and communication steps required by FTTE and other baselines - FedAVG, AsyncFL, and FedBuff to achieve target accuracy on different model architectures - MCUNet, MobileNetV2, and ProxylessNAS. The results span 4 different datasets distributed across 100 clients with 50\% stragglers using a Dirichlet distribution $\alpha=100000$ indicating homogenous (IID) data distribution.}
\label{iid}
\resizebox{1\columnwidth}{!}{%
\begin{tabular}{cccccc}
\hline
\multicolumn{6}{c}{\cellcolor[HTML]{EFEFEF}\textbf{MCUNet}} \\ \hline
 & \textbf{Target Acc.} & \textbf{FedAVG} & \textbf{AsyncFL} & \textbf{FedBuff} & \textbf{FTTE (Ours)} \\ \hline
Skin Cancer & 50.1\% & 6000 ($\times$5.04) & >10k(>8.41) & 3443 ($\times$2.89) & 1189 \\
\rowcolor[HTML]{F5F5F5} 
CIFAR-10 & 73.1\% & 5000 ($\times$7.09) & >10k(>14.18) & 1497 ($\times$2.12) & 705 \\
Oxford-PETS & 58.23\% & 5000 ($\times$3.98) & >10k(>7.97) & >10k(>$\times$7.97) & 1255 \\
\rowcolor[HTML]{F5F5F5} 
Flowers-102 & 51.8\% & 6600 ($\times$5.45) & >10k(>8.25) & >10k(>$\times$8.25) & 1211 \\ \hline
\multicolumn{6}{c}{\cellcolor[HTML]{EFEFEF}\textbf{MobileNetV2}} \\ \hline
 & \textbf{Target Acc.} & \textbf{FedAVG} & \textbf{AsyncFL} & \textbf{FedBuff} & \textbf{FTTE (Ours)} \\ \hline
Skin Cancer & 50.20\% & 5800 ($\times$5.85) & >10k(>10.09) & 2591 ($\times$2.61) & 991 \\
\rowcolor[HTML]{F5F5F5} 
CIFAR-10 & 70.1\% & 4600 ($\times$6.73) & >10k(>14.64) & >10k (>$\times$14.64) & 683 \\
Oxford-PETS & 54.1\% & 4400 ($\times$4.87) & >10k(>11.07) & >10k (>$\times$11.07) & 903 \\
\rowcolor[HTML]{F5F5F5} 
Flowers-102 & 45.3\% & 4200 ($\times$3.81) & Osc. & >10k ($\times$9.08) & 1101 \\ \hline
\multicolumn{6}{c}{\cellcolor[HTML]{EFEFEF}\textbf{ProxylessNAS}} \\ \hline
 & \textbf{Target Acc.} & \textbf{FedAVG} & \textbf{AsyncFL} & \textbf{FedBuff} & \textbf{FTTE (Ours)} \\ \hline
Skin Cancer & 48.91\% & 5800 ($\times$6.75) & >10k (>$\times$11.64) & 3179 ($\times$3.7)) & 859 \\
\rowcolor[HTML]{F5F5F5} 
CIFAR-10 & 71.9\% & 3800 ($\times$5.95) & Osc. & >10k (>$\times$15.65) & 639 \\
Oxford-PETS & 58.6\% & 4600 ($\times$4.18) & Osc. & >10k (>$\times$9.08) & 1101 \\
\rowcolor[HTML]{F5F5F5} 
Flowers-102 & 53.8\% & 6200 ($\times$4.40) & >10k (>$\times$7.09) & 1541 ($\times$1.09)  & 1409 \\ \hline
\end{tabular}%
}
\end{table}


==> tables/table4.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\begin{tabular}{lccccc}
\hline
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}\textbf{Model}} & \textbf{Algorithm}                                     & \textbf{Flowers-102}    & \textbf{Oxford Pets}    & \textbf{CIFAR-10}       & \textbf{Skin Cancer}    \\ \hline
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{FFFFFF}                                   & \begin{tabular}[c]{@{}c@{}}Target \\ Acc.\end{tabular} & 51.8 \%                 & 58.3 \%                 & 72 \%                   & 49.57 \%                \\ \cline{2-6} 
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}                                   & \textbf{FedAVG}                                        & 6600 (x5.45)            & 5000 (x3.98)            & 5000 (x7.09)            & 6000 (x5.04)            \\
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{FFFFFF}                                   & \textbf{AsyncFL}                                       &                         &                         &                         &                         \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}                                   & \textbf{FedBuff}                                       & >10k (>x8.26)           & >10k (>x7.96)           & >10k (>x14.18)          & >10k (>x8.41))          \\
\rowcolor[HTML]{EFEFEF} 
\multirow{-5}{*}{\cellcolor[HTML]{FFFFFF}MCUNet}           & \textbf{FTTE (Ours)}                                   & 1211                    & 1255                    & 705                     & 1189                    \\ \hline
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}                                   & \begin{tabular}[c]{@{}c@{}}Target \\ Acc.\end{tabular} & 50.5 \%                 & 53.4 \%                 & 70.3 \%                 & 46.4 \%                 \\ \cline{2-6} 
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{FFFFFF}                                   & \textbf{FedAVG}                                        & 5000 (x4.45)            & 3400 (x4.06)            & 4800 (x4.95)            & 5600 (x5.30)            \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}                                   & {\color[HTML]{333333} \textbf{AsyncFL}}                & {\color[HTML]{333333} } & {\color[HTML]{333333} } & {\color[HTML]{333333} } & {\color[HTML]{333333} } \\
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{FFFFFF}                                   & \textbf{FedBuff}                                       & >10k (>x8.90)           &                         &                         & >10k (>x9.46)           \\
\rowcolor[HTML]{FFFFFF} 
\multirow{-5}{*}{\cellcolor[HTML]{FFFFFF}MobileNetV2}      & \textbf{FTTE (Ours)}                                   & 1123                    & 837                     & 969                     & 1057                    \\ \hline
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{FFFFFF}                                   & \begin{tabular}[c]{@{}c@{}}Target \\ Acc.\end{tabular} & 50.5 \%                 & 53.4 \%                 & 70.30 \%                & 46.4 \%                 \\ \cline{2-6} 
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}                                   & \textbf{FedAVG}                                        & 5000 (x4.45)            & 3400 (x4.06)            & 4800 (x4.95)            & 5600 (x5.30)            \\
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{FFFFFF}                                   & \textbf{AsyncFL}                                       & Osc.                    & Osc.                    & >10k (>x10.31)          & >10k (>x9.4)            \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}                                   & \textbf{FedBuff}                                       & 1475 (x1.31)            & 3153 (x3.77)            & >10k (>x10.31)          & 2651 (x2.51)            \\
\rowcolor[HTML]{EFEFEF} 
\multirow{-5}{*}{\cellcolor[HTML]{FFFFFF}ProxylessNAS}     & \textbf{FTTE (Ours)}                                   & 1123                    & 837                     & 969                     & 1057                    \\ \hline
\end{tabular}
\end{table}

==> tables/table4_v2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\caption{Target accuracy and communication steps required by FTTE and other baselines - FedAVG, AsyncFL, and FedBuff to achieve target accuracy on different model architectures - MCUNet, MobileNetV2, and ProxylessNAS. The results span 4 different datasets distributed across 100 clients with 50\% stragglers using a Dirichlet distribution $\alpha=1.0$ indicating moderately heterogenous data distribution.}
\label{med_iid}
\resizebox{1\columnwidth}{!}{%
\begin{tabular}{cccccc}
\hline
\multicolumn{6}{c}{\cellcolor[HTML]{EFEFEF}\textbf{MCUNet}} \\ \hline
 & \textbf{Target Acc.} & \textbf{FedAVG} & \textbf{AsyncFL} & \textbf{FedBuff} & \textbf{FTTE (Ours)} \\ \hline
Skin Cancer & 49.57\% & 6000 ($\times$5.04) & >10k (>$\times$8.41 & >10k (>$\times$8.41) & 1189 \\
\rowcolor[HTML]{F5F5F5} 
CIFAR-10 & 72\% & 5000 ($\times$7.09) & Osc. & >10k (>$\times$14.18) & 705 \\
Oxford-PETS & 58.3\% & 5000 ($\times$3.98) & Osc. & >10k (>$\times$7.96) & 1255 \\
\rowcolor[HTML]{F5F5F5} 
Flowers-102 & 51.8\% & 6600 ($\times$5.45) & >10k (>$\times$8.26) & >10k (>$\times$8.26) & 1211 \\ \hline
\multicolumn{6}{c}{\cellcolor[HTML]{EFEFEF}\textbf{MobileNetV2}} \\ \hline
 & \textbf{Target Acc.} & \textbf{FedAVG} & \textbf{AsyncFL} & \textbf{FedBuff} & \textbf{FTTE (Ours)} \\ \hline
Skin Cancer & 46.4\% & 5600 ($\times$5.30) & Osc. & >10k (>$\times$9.46) & 1057 \\
\rowcolor[HTML]{F5F5F5} 
CIFAR-10 & 70.3\% & 4800 ($\times$4.95) & >10k (>10.32) & >10k (>10.32) & 969 \\
Oxford-PETS & 53.4\% & 3400 ($\times$4.06) & >10k (11.95) & Osc. & 837 \\
\rowcolor[HTML]{F5F5F5} 
Flowers-102 & 50.5\% & 5000 ($\times$4.45) & Osc. & >10k (>$\times$8.90) & 1123 \\ \hline
\multicolumn{6}{c}{\cellcolor[HTML]{EFEFEF}\textbf{ProxylessNAS}} \\ \hline
 & \textbf{Target Acc.} & \textbf{FedAVG} & \textbf{AsyncFL} & \textbf{FedBuff} & \textbf{FTTE (Ours)} \\ \hline
Skin Cancer & 46.4\% & 5600 ($\times$5.30) & >10k (>$\times$9.46) & 2651 ($\times$2.51) & 1057 \\
\rowcolor[HTML]{F5F5F5} 
CIFAR-10 & 70.30\% & 4800 ($\times$4.95) & >10k (>$\times$10.31) & >10k (>$\times$10.31) & 969 \\
Oxford-PETS & 53.4\% & 3400 ($\times$4.06) & Osc. & 3153 ($\times$3.77) & 837 \\
\rowcolor[HTML]{F5F5F5} 
Flowers-102 & 50.5\% & 5000 ($\times$4.45) & Osc. & 1475 ($\times$1.31) & 1123 \\ \hline
\end{tabular}%
}
\end{table}


==> tables/table5.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\begin{tabular}{lccccc}
\hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{c}{\cellcolor[HTML]{EFEFEF}\textbf{Model}} & \textbf{Algorithm}                                     & \textbf{Flowers-102}                                & \textbf{Oxford Pets}                              & \textbf{CIFAR-10}                                    & \textbf{Skin Cancer}                                 \\ \hline
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}                                   & \begin{tabular}[c]{@{}c@{}}Target \\ Acc.\end{tabular} & 41.82 \%                                            & 48.64 \%                                          & 61.63 \%                                             & 44.67 \%                                             \\ \cline{2-6} 
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{FFFFFF}                                   & \textbf{FedAVG}                                        & 6600 (x4.41)                                        & 5000 (x3.49)                                      & 5000 (x3.49)                                         & 6000 (x2.78)                                         \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}                                   & \textbf{AsyncFL}                                       &                                                     &                                                   &                                                      &                                                      \\
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{FFFFFF}                                   & \textbf{FedBuff}                                       & >10k (>x6.68)                                       & Osc.                                              & >10k (>x6.99)                                        & Osc.                                                 \\
\rowcolor[HTML]{FFFFFF} 
\multirow{-5}{*}{\cellcolor[HTML]{FFFFFF}MCUNet}           & \cellcolor[HTML]{FFFFFF}\textbf{FTTE (Ours)}           & 1497                                                & 1434                                              & 1431                                                 & 2157                                                 \\ \hline
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{FFFFFF}                                   & \begin{tabular}[c]{@{}c@{}}Target \\ Acc.\end{tabular} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}39.8 \%} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}46 \%} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}57.87 \%} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}39.53 \%} \\ \cline{2-6} 
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}                                   & \textbf{FedAVG}                                        & 4400 (x3.27)                                        & 5000 (x3.78)                                      & 3000 (x4.26)                                         & 3200 (x2.59)                                         \\
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{FFFFFF}                                   & \textbf{AsyncFL}                                       &                                                     &                                                   &                                                      &                                                      \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}                                   & \textbf{FedBuff}                                       & >10k (>x7.45)                                       & >10k (>x7.57)                                     &                                                      & 2761 (x2.24)                                         \\
\rowcolor[HTML]{EFEFEF} 
\multirow{-5}{*}{\cellcolor[HTML]{FFFFFF}MobileNetV2}      & \textbf{FTTE (Ours)}                                   & 1343                                                & 1321                                              & 705                                                  & 1233                                                 \\ \hline
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}                                   & \begin{tabular}[c]{@{}c@{}}Target \\ Acc.\end{tabular} & 43.90 \%                                            & 45.9 \%                                           & 60.7 \%                                              & 38.17 \%                                             \\ \cline{2-6} 
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{FFFFFF}                                   & \textbf{FedAVG}                                        & 5000 (x3.5)                                         & 4500 (x4.26)                                      & 3800 (x2.93)                                         & 2800 (x3.35)                                         \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}                                   & \textbf{AsyncFL}                                       & Osc.                                                & Osc.                                              & Osc.                                                 & Osc.                                                 \\
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{FFFFFF}                                   & \textbf{FedBuff}                                       & 1717 (x1.2)                                         & 1421 (x1.34)                                      & Osc.                                                 & >10k (>11.94)                                        \\
\rowcolor[HTML]{FFFFFF} 
\multirow{-5}{*}{\cellcolor[HTML]{FFFFFF}ProxylessNAS}     & \textbf{FTTE (Ours)}                                   & 1431                                                & 1057                                              & 1299                                                 & 837                                                  \\ \hline
\end{tabular}
\end{table}

==> tables/table5_v2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\caption{Target accuracy and communication steps required by FTTE and other baselines - FedAVG, AsyncFL, and FedBuff to achieve target accuracy on different model architectures - MCUNet, MobileNetV2, and ProxylessNAS. The results span 4 different datasets distributed across 100 clients with 50\% stragglers using a Dirichlet distribution $\alpha=0.1$ indicating heterogenous data distribution.}
\label{non-iid}
\resizebox{1\columnwidth}{!}{%
\begin{tabular}{cccccc}
\hline
\multicolumn{6}{c}{\cellcolor[HTML]{EFEFEF}\textbf{MCUNet}} \\ \hline
 & \textbf{Target Acc.} & \textbf{FedAVG} & \textbf{AsyncFL} & \textbf{FedBuff} & \textbf{FTTE (Ours)} \\ \hline
Skin Cancer & 44.67\% & 6000 ($\times$2.78) & Osc. & Osc. & 2157 \\
\rowcolor[HTML]{F5F5F5}
CIFAR-10 & 61.63\% & 5000 ($\times$3.49) & Osc. & >10k (>$\times$6.99) & 1431 \\
Oxford-PETS & 48.64\% & 5000 ($\times$3.49) & Osc. & Osc. & 1434 \\
\rowcolor[HTML]{F5F5F5}
Flowers-102 & 41.82\% & 6600 ($\times$4.41) & Osc. & >10k (>$\times$6.68) & 1497 \\ \hline
\multicolumn{6}{c}{\cellcolor[HTML]{EFEFEF}\textbf{MobileNetV2}} \\ \hline
 & \textbf{Target Acc.} & \textbf{FedAVG} & \textbf{AsyncFL} & \textbf{FedBuff} & \textbf{FTTE (Ours)} \\ \hline
Skin Cancer & 39.53\% & 3200 ($\times$2.59) & Osc. & 2761 ($\times$2.24) & 1233 \\
\rowcolor[HTML]{F5F5F5}
CIFAR-10 & 57.87\% & 3000 ($\times$4.26) & Osc. & Osc. & 705 \\
Oxford-PETS & 46\% & 5000 ($\times$3.78) & Osc. & >10k (>$\times$7.57) & 1321 \\
\rowcolor[HTML]{F5F5F5}
Flowers-102 & 39.8\% & 4400 ($\times$3.27) & Osc. & >10k (>$\times$7.45) & 1343 \\ \hline
\multicolumn{6}{c}{\cellcolor[HTML]{EFEFEF}\textbf{ProxylessNAS}} \\ \hline
 & \textbf{Target Acc.} & \textbf{FedAVG} & \textbf{AsyncFL} & \textbf{FedBuff} & \textbf{FTTE (Ours)} \\ \hline
Skin Cancer & 38.17\% & 2800 ($\times$3.35) & Osc. & >10k (>11.94) & 837 \\
\rowcolor[HTML]{F5F5F5}
CIFAR-10 & 60.7\% & 3800 ($\times$2.93) & Osc. & Osc. & 1299 \\
Oxford-PETS & 45.9\% & 4500 ($\times$4.26) & Osc. & 1421 ($\times$1.34) & 1057 \\
\rowcolor[HTML]{F5F5F5}
Flowers-102 & 43.90\% & 5000 ($\times$3.5) & Osc. & 1717 ($\times$1.2) & 1431 \\ \hline
\end{tabular}%
}
\end{table}


==> tables/table6.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\caption{Target accuracy and communication steps required by FTTE with Adam optimizer (as local optimizer) and FedAdam \cite{reddi2021adaptivefederatedoptimization} to achieve target accuracy on MCUNet with different datasets and data distributions. This Federated network consists of 100 clients with 50\% stragglers.}
\label{adaptive}
\resizebox{0.65\columnwidth}{!}{%
\begin{tabular}{ccccc}
\hline
\multicolumn{5}{c}{\cellcolor[HTML]{EFEFEF}\textbf{MCUNet}}                                                                                                                                                                                                                                                                                                                           \\ \hline
\multicolumn{1}{l}{}                                                                          &                                                    &                                                                                  &                                                            &                                                                                            \\
\multicolumn{1}{l}{\multirow{-2}{*}{}}                                                        & \multirow{-2}{*}{\textbf{$\alpha$}}                & \multirow{-2}{*}{\textbf{Target Acc.}} & \multirow{-2}{*}{\textbf{FedAdam}}                         & \multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}FTTE (Ours)\\ with Adam\end{tabular}}} \\ \hline
                                                                                              & \cellcolor[HTML]{F5F5F5}100000                     & \cellcolor[HTML]{F5F5F5}45.67\%                                                    & \cellcolor[HTML]{F5F5F5}6200 ($\times$7.6)                        & \cellcolor[HTML]{F5F5F5}815                                                                \\
                                                                                              & 1.0                                                & 43.70\%                                                                            & 4400 ($\times$3.5)                                                & 1269                                                                                       \\
\multirow{-3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Skin Cancer\\ (8 classes)\end{tabular}}}  & \cellcolor[HTML]{F5F5F5}{\color[HTML]{000000} 0.1} & \cellcolor[HTML]{F5F5F5}{\color[HTML]{333333} 30.05\%}                             & \cellcolor[HTML]{F5F5F5}{\color[HTML]{333333} 2600 ($\times$2.7)} & \cellcolor[HTML]{F5F5F5}{\color[HTML]{333333} 969}                                         \\ \hline
                                                                                              & 100000                                             & 67.46\%                                                                            & 9200 ($\times$7.6)                                                & 1211                                                                                       \\
                                                                                              & \cellcolor[HTML]{F5F5F5}1.0                        & \cellcolor[HTML]{F5F5F5}63.57\%                                                    & \cellcolor[HTML]{F5F5F5}8000 ($\times$6.7)                        & \cellcolor[HTML]{F5F5F5}1300                                                               \\
\multirow{-3}{*}{\textbf{CIFAR-10}}                                                           & 0.1                                                & 50.70\%                                                                            & 6600 ($\times$5.2)                                                & 1267                                                                                       \\ \hline
                                                                                              & \cellcolor[HTML]{F5F5F5}100000                     & \cellcolor[HTML]{F5F5F5}67.34\%                                                    & \cellcolor[HTML]{F5F5F5}4800 ($\times$4.2)                        & \cellcolor[HTML]{F5F5F5}1135                                                               \\
                                                                                              & 1.0                                                & 66.02\%                                                                            & 3665 ($\times$4.5)                                                & 815                                                                                        \\
\multirow{-3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Oxford-PETS\\ (37 classes)\end{tabular}}} & \cellcolor[HTML]{F5F5F5}0.1                        & \cellcolor[HTML]{F5F5F5}56.02\%                                                    & \cellcolor[HTML]{F5F5F5}2900 ($\times$1.5)                        & \cellcolor[HTML]{F5F5F5}1915                                                               \\ \hline
                                                                                              & 100000                                             & 67.28\%                                                                            & 5400 ($\times$5.3)                                                & 1017                                                                                       \\
                                                                                              & \cellcolor[HTML]{F5F5F5}1.0                        & \cellcolor[HTML]{F5F5F5}65.69\%                                                    & \cellcolor[HTML]{F5F5F5}5000 ($\times$4.5)                        & \cellcolor[HTML]{F5F5F5}1101                                                               \\
\multirow{-3}{*}{\textbf{Flowers-102}}                                                        & 0.1                                                & 64.56\%                                                                            & 6900 ($\times$3.5)                                                & 1981                                                                                       \\ \hline
\end{tabular}}
\end{table}

==> tables/table7.tex <==

\begin{tabular}{clcc}
\hline
                                                                        &                                                 & \textbf{\begin{tabular}[c]{@{}c@{}}Target\\ Acc.\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Comm.\\ Steps\end{tabular}} \\ \hline
                                                                        & \cellcolor[HTML]{EFEFEF}$1/(1+age)$             & \cellcolor[HTML]{EFEFEF}58.42 \%                               & \cellcolor[HTML]{EFEFEF}1157                                   \\
                                                                        & $1/(1+age)^2$                                   & 53.65 \%                                                       & 995                                                            \\
\multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Oxford\\ Pets\end{tabular}} & \cellcolor[HTML]{EFEFEF}$1/(1+age*Var.)$   & \cellcolor[HTML]{EFEFEF}58.30 \%                                   & \cellcolor[HTML]{EFEFEF}925                                    \\ \hline
                                                                        & \cellcolor[HTML]{EFEFEF}$1/(1+age)$             & \cellcolor[HTML]{EFEFEF}70.50 \%                                & \cellcolor[HTML]{EFEFEF}881                                    \\
                                                                        & $1/(1+age)^2$                                   & 68.77 \%                                                       & 897                                                            \\
\multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}CIFAR\\ 10\end{tabular}}    & \cellcolor[HTML]{EFEFEF}$1/(1+age*Var.)$   & \cellcolor[HTML]{EFEFEF}72.21 \%                               & \cellcolor[HTML]{EFEFEF}771                                    \\ \hline
\end{tabular}

